Taming False Positives in Out-of-Distribution Detection with Human Feedback

Robustness to out-of-distribution (OOD) samples is crucial for safely deploying machine learning models in the open world. Recent works have focused on designing scoring functions to quantify OOD uncertainty. Setting appropriate thresholds for these scoring functions for OOD detection is challenging as OOD samples are often unavailable up front. Typically, thresholds are set to achieve a desired true positive rate (TPR), e.g., $95\%$ TPR. However, this can lead to very high false positive rates (FPR), ranging from 60 to 96\%, as observed in the Open-OOD benchmark. In safety-critical real-life applications, e.g., medical diagnosis, controlling the FPR is essential when dealing with various OOD samples dynamically. To address these challenges, we propose a mathematically grounded OOD detection framework that leverages expert feedback to \emph{safely} update the threshold on the fly. We provide theoretical results showing that it is guaranteed to meet the FPR constraint at all times while minimizing the use of human feedback. Another key feature of our framework is that it can work with any scoring function for OOD uncertainty quantification. Empirical evaluation of our system on synthetic and benchmark OOD datasets shows that our method can maintain FPR at most $5\%$ while maximizing TPR.

==> sections/LIL.tex <==
First assume that $\gamma$ is constant and there is no shift in the distributions or their mixtures. The algorithm will query labels for all points till some time point $T_0$ to have accurate estimates of $\FPR(\lambda,T_0)$ and $\TPR(\lambda,T_0)$ for all $\lambda \in \Lambda$, so that it can satisfy the $\FPR$ constraint while having non-trivial $\TPR$.



==> sections/algo_2.tex <==
%\vspace{-10pt}

\begin{wrapfigure}{r}{0.5\textwidth}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\caption{ SolveOptForLambda} \label{alg:solve-lambda}
\Require{FPR threshold $\alpha$ , window size $N_w$, $S_t, L_t, I_t, \nu>0$
%}\Statex{ $\hspace{11pt}$  


%\Ensure{x}
\State $k = \lceil\frac{\Lambda_{\max}-\Lambda_{\min}}{\nu} \rceil$ 
\State {$\lambda_a = \Lambda_{\min}+\nu \cdot a \quad \forall a \in {0,\ldots, k}$}
\State {$a_{\min} = 0 $, $a_{\max} = k$}
\For{  $j = 0,1,\ldots k$ }
   \State{$a_{mid} = \lceil\frac{a_{\min}+a_{\max}}{2} \rceil$}
   \State{$\lambda_{mid} = \lambda_{a_{mid}}$}
   \State{
   $O_t = \{ u\le t:  y_t=-1, l_t=1 \}$}
   \State{ Let $O_t'$ be set of indices the most recent $N_w$ OOD points.}
   \State{
   $m_a = \sum_{u\in O_t': i_u=0 }\mathbf{1}(s_u \ge \lambda_{mid})$}
   
   \State{$m_b = \sum_{u\in O_t': i_u=1 }\mathbf{1}(s_u \ge \lambda_{mid})$}
    \State{$\FPRhat(\lambda_{mid},t) = \frac{1}{|O_t'|} \Big ( m_a + \frac{1}{p}m_b \Big )$}
    \State{ Compute $\psi(t)$ as in equation \eqref{eqn:psi-theory}}
    
   \If{ $ \FPRhat(\lambda_{mid},t) + \psi(t) \le \alpha$}
   \State{$a_{\max}=a_{mid}$}
   \Else 
      \State{$ a_{\min} = a_{mid}$}
   \EndIf
\EndFor
\State {Output $\lambda_{mid}$}
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

==> sections/algo_2_short.tex <==
%\vspace{-pt}
%\begin{wrapfigure}{r}
%{0.5\textwidth}
%\begin{minipage}{0.5\textwidth}
\vspace{-20pt}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\caption{ SolveOptForLambda} \label{alg:solve-lambda}
\Require{FPR threshold $\alpha$ , $S_t$, $N_w$}
%}\Statex{ $\hspace{11pt}$  
\State{
%\begin{aligned}
%\vspace{-10pt}
\begin{align*}
\hat{\lambda}_t := \text{arg } \underset{\lambda  \in \Lambda}{\text{min}}\ \lambda\ \text{ s.t. }\ \FPRhat(\lambda,t) + \psi(t,\delta)\le \alpha 
%\vspace{-25pt}
\end{align*} }
\State{ Output $\hat{\lambda}_t$}
\end{algorithmic}
\end{algorithm}
\vspace{-15pt}
%\end{minipage}
%\end{wrapfigure}
